Canonical Quantization of Superconducting Circuits

In the quest to produce quantum technology, superconducting networks, working at temperatures just above absolute zero, have arisen as one of the most promising physical implementations. The precise analysis and synthesis of such circuits have required merging the fields of physics, engineering, and mathematics. In this dissertation, we develop mathematically consistent and precise Hamiltonian models to describe ideal superconducting networks made of an arbitrary number of lumped elements, such as capacitors, inductors, Josephson and phase-slip junctions, gyrators, etc., and distributed ones like transmission lines. We give formal proofs for the decoupling at high and low frequencies of lumped degrees of freedom from infinite-dimensional systems in different coupling configurations in models based on the effective Kirchhoff's laws. We extend the standard theory to quantize circuits that include ideal nonreciprocal elements all the way to their Hamiltonian descriptions in a systematic way. Finally, we pave the way on how to quantize general frequency-dependent gyrators and circulators coupled to both transmission lines and other lumped-element networks. We have explicitly shown, that these models, albeit ideal, are finite and present no divergence issues. We explain and dispel misunderstandings from the previous literature. Furthermore, we have demonstrated the usefulness of a redundant basis for performing separation of variables of the transmission line (1D) fields in the presence of point-like (lumped-element) couplings by time-reversal symmetry-breaking terms, i.e. nonreciprocal elements.

==> misc/dedicatoria2.tex <==
\thispagestyle{empty}


\vspace*{5cm}
\begin{flushright}
{\emph{{To those who inspired my quest 
}}}
\end{flushright}


==> others/prologue.tex <==
\addcontentsline{toc}{section}{Prologue}
\chapter*{Prologue}

\textbf{This is a Prologue. May I write one?}\\\\
The work presented in this Ph.D. thesis explores different gravitational, observational and cosmological properties of large volume-complete samples of massive clusters of galaxies drawn from different photometric cluster catalogues constructed from Sloan Digital Sky Survey (SDSS) data. It is based on different projects made in collaboration with my supervisors Tom Broadhurst and Ruth Lazkoz, and my collaborators, Jose Maria Diego, Keiichi Umetsu, Jean Coupon, Raul Angulo and Ivan De Martino.

Clusters of galaxies, the most massive gravitationally bound structures in the Universe, are one of the most important probes to constrain cosmological models. 
Located at the peaks of the underlying large scale matter distribution, their number density and spatial clustering as a function of halo mass and redshift may shed light on some of the most profound mysteries of modern cosmology and physics in general, like the origin of the present accelerated expansion of the Universe, or the nature of dark matter. 
Also, the evolutionary dynamics of clusters and the effects produced by their deep gravitational potential wells provide us with unique tools to discriminate between different theories of gravity.

New and ongoing surveys at mm, near-infrared, optical and X-ray wavelengths have the potential to locate hundreds of thousands of clusters in the sky. 
However, the real challenge for cluster cosmology is not the identification of clusters, but the accurate calibration of the relation between cluster mass and the observational proxies used to estimate it, which often involve complicated baryonic physics.

In Part~\ref{part_1} of this thesis some basic concepts of modern cosmology are introduced, together with the theory of growth of structures that lets us link the present-day large scale structure of the Universe with the primordial perturbations originated shortly after the \textit{Big Bang}.
We then describe some of the physics associated to clusters of galaxies, including the effects whose origin is found in the strong curvature of space-time generated by these extremely massive systems, and the distortion introduced in the spectra of the cosmic microwave background photons, known as Sunyaev-Zel'dovich effect, when these interact with the energetic free electrons of the intracluster medium. Because it is one of the main objectives of this work, we also summarize how to statistically relate the number of galaxies contained in clusters to the total mass. In the last part of the introduction we describe the SDSS and the cluster catalogues that we consider in our analyses.

The original results obtained during the Ph.D. research period are presented in Part~\ref{part_2}. First, in Chap.~\ref{chapter:chapter_4}, we measure the gravitational redshift and redshift enhancement effects considering three different cluster catalogues constructed from SDSS data, namely the GMBCG, WHL12 and redMaPPer cluster catalogues, and study the dependence of the amplitude of these effects with cluster mass, in order to understand the results obtained. This chapter is based on the published work:
\begin{itemize}
 \item \PublicationEntry{Comparing gravitational redshifts of SDSS galaxy clusters with the magnified redshift enhancement of background BOSS galaxies}{P. Jimeno, T. Broadhurst, J. Coupon, K. Umetsu, R. Lazkoz}{MNRAS, 448, 1999 (2015). \href{http://adsabs.harvard.edu/abs/2015MNRAS.448.1999J}{arXiv:1410.6050}}
\end{itemize}

\vspace{-5pt}

In Chap.~\ref{chapter:chapter_5} and focusing efforts on the redMaPPer catalogue, which we previously update with the most recent SDSS spectroscopic data, we study the mass and redshift dependence of the number density and spatial clustering of different samples of clusters binned in richness and redshift. In the second part of this chapter we constrain the parameters of the mass--richness relation comparing our measurements with those provided by the Millennium-XXL (MXXL) cosmological $N$-body simulation, from which we construct synthetic cluster samples. The results obtained in this chapter were published in the paper:
\begin{itemize}
\item \PublicationEntry{Precise clustering and density evolution of redMaPPer galaxy clusters versus MXXL simulation}{P. Jimeno, T. Broadhurst, R. Lazkoz, R. Angulo, J.-M. Diego, K. Umetsu, M.-c. Chu}{MNRAS, 466, 2658 (2017). \href{http://adsabs.harvard.edu/abs/2017MNRAS.466.2658J}{arXiv:1608.05446}}
\end{itemize}

\vspace{-5pt}

Finally, in Chap.~\ref{chapter:chapter_6} we study the Sunyaev-Zel'dovich effect signal coming from 6 different richness subsamples of redMaPPer clusters. To do so, we construct our own Compton parameter maps using data from the space satellite \textit{Planck}. Through Bayesian Markov chain Monte Carlo (MCMC) techniques, we first constrain the parameters that describe the pressure profile of clusters, and then obtain an estimate of the mass bias and of the mass--richness relation comparing our results with results based on weak lensing. The methodology and results described in this chapter can be found at:
\begin{itemize}
 \item \PublicationEntry{\textit{Planck}/SDSS Cluster Mass and Gas Scaling Relations for a Volume-Complete redMaPPer Sample}{P. Jimeno, J.-M. Diego, T. Broadhurst, I. De Martino, R. Lazkoz}
{Submitted to MNRAS \href{https://arxiv.org/abs/1706.00395}{arXiv:1706.00395}}
\end{itemize}


